Per-Domain Generalizing Policies: On Validation Instances and Scaling Behavior

Recent work has shown that successful per-domain generalizing action policies can be learned. Scaling behavior, from small training instances to large test instances, is the key objective; and the use of validation instances larger than training instances is one key to achieve it. Prior work has used fixed validation sets. Here, we introduce a method generating the validation set dynamically, on the fly, increasing instance size so long as informative and feasible.We also introduce refined methodology for evaluating scaling behavior, generating test instances systematically to guarantee a given confidence in coverage performance for each instance size. In experiments, dynamic validation improves scaling behavior of GNN policies in all 9 domains used.

==> gnn.tex <==
\section{Relational Graph Neural Network}
\label{gnn}
Before introducing the newly proposed evaluation, we briefly explain the GNN architecture used throughout this paper. 
We use  \citeauthor{staahlberg2022learning}'s relational graph neural network (RGNN)~\cite{staahlberg2022learning,staahlberg2024learning}. 
However, we do not use the same policies, but use that architecture to train new general policies. 


For a fixed domain, the relational GNN is trained to compute a \emph{state value function} $V$, which, given a state $s$ from any instance, returns the optimal cost $V(s)$ for reaching a goal state from $s$.
The learned value function $V$ then induces a policy if, for any given state $s$, we always transition to the successor state $s'$ with the lowest state value $V(s')$.

The relational GNN consists of several multi-layer perceptrons (MLP): A predicate MLP$_{p}$ for each predicate $p$, an update MLP$_{U}$, a readout MLP$_{R}$, and output MLP$_{O}$. 
%We will refer to them as $\mathbf{MLP}_{p}$, $\mathbf{MLP}_{U}$, $\mathbf{MLP}_{R}$, and $\mathbf{MLP}_{O}$, respectively, and explain their functions in the following.
Given a state $s$, the relational GNN computes an embedding $h(o)$ for each object $o$ in the instance, which are then used to predict $V(s)$.
The object embeddings $h(o)$ are computed iteratively, where the initial embeddings $h_{0}(o)$ only contain zeros.
Every iteration $i$ consists of two steps:
\begin{enumerate}
	\item \emph{Message Computation}: For each atom $q = p(o_{1}, ...,  o_{n})$ true in $s$, the involved objects' embeddings $h_{i}(o)$ are passed to MLP$_{p}$, which computes a so-called message $m_{q}$.
	\item \emph{Embedding Update}: %For each object $o$, the messages $m_{q}$ with $o \in q$ are aggregated into an object-specific message $m_{o}$. The new embedding $h_{i+1}(o)$ is then computed by passing $h_{i}(o)$ and $m_{o}$ to MLP$_{U}$.
	For each object $o$, we aggregate the messages $m_{q}$ with $o \in q$ into an object-specific message $m_{o}$ by taking a dimension-wise maximum. The new embedding $h_{i+1}(o)$ is then computed by passing $h_{i}(o)$ and $m_{o}$ to MLP$_{U}$.
\end{enumerate}
After $L$ iterations, we aggregate the object embeddings $h_{L}(o)$ into a single state embedding $h(s)$ using a readout operation. Here, we first pass each $h_{L}(o)$ to MLP$_{R}$ and then compute a dimension-wise sum. Lastly, the state embedding $h(s)$ is given to MLP$_{O}$, which outputs $V(s)$.
\nicola{No pseudocode for GNN to save space?}
\nicola{Well... do we even need to explain the GNN?}
\tg{to understand this, a figure would help a lot. @joerg what do you think? yes, no, or yes but only in appendix? We could also refer to the original paper for details}

%For example, consider a state of a Blocksworld instance where the only true atoms are $q_{1}=on(a, b)$ and $q_{2}=on(b,c)$. 

